Channel Charting-Based Channel Prediction on Real-World Distributed Massive MIMO CSI

Distributed massive MIMO is considered a key advancement for improving the performance of next-generation wireless telecommunication systems. However, its efficacy in scenarios involving user mobility is limited due to channel aging. To address this challenge, channel prediction techniques are investigated to forecast future channel state information (CSI) based on previous estimates. We propose a new channel prediction method based on channel charting, a self-supervised learning technique that reconstructs a physically meaningful latent representation of the radio environment using similarity relationships between CSI samples. The concept of inertia within a channel chart allows for predictive radio resource management tasks through the latent space. We demonstrate that channel charting can be used to predict future CSI by exploiting spatial relationships between known estimates that are embedded in the channel chart. Our method is validated on a real-world distributed massive MIMO dataset, and compared to a Wiener predictor and the outdated CSI in terms of achievable sum rate.

==> fig/sum_rate_old.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={prediction horizon \(\displaystyle p\)},
xmajorgrids,
xmin=-1.25, xmax=26.25,
xtick style={color=black},
y grid style={darkgray176},
ylabel={$\mathrm{SR} \left(\si{bit\per s\per \hertz}\right)$},
ymajorgrids,
ymin=115.088628005981, ymax=172.226717758179,
ytick style={color=black}
]
\addplot [thick, steelblue31119180, mark=*, mark size=1, mark options={solid}]
table {%
0 169.629531860352
1 161.069259643555
2 151.698959350586
3 149.069854736328
4 147.341781616211
5 144.751190185547
6 141.07487487793
7 138.786178588867
8 136.987228393555
9 134.6083984375
10 132.161102294922
11 130.759994506836
12 128.860946655273
13 126.618583679199
14 124.82300567627
15 124.108955383301
16 123.513511657715
17 122.578590393066
18 121.538619995117
19 120.831481933594
20 120.193000793457
21 119.63591003418
22 118.953338623047
23 118.675323486328
24 118.406135559082
25 117.685813903809
};
\addlegendentry{$\mathbf{\hat{H}}_\mathrm{outdated}'$}
\addplot [thick, darkorange25512714, mark=*, mark size=1, mark options={solid}]
table {%
0 152.041030883789
1 150.484481811523
2 149.18359375
3 147.945159912109
4 146.785842895508
5 145.740005493164
6 144.703567504883
7 143.969696044922
8 143.311294555664
9 142.247283935547
10 141.117858886719
11 140.628036499023
12 139.495971679688
13 138.885330200195
14 137.865188598633
15 137.57389831543
16 137.143341064453
17 136.271011352539
18 135.864212036133
19 135.039764404297
20 133.965606689453
21 133.222259521484
22 132.646408081055
23 132.24690246582
24 131.556625366211
25 130.889099121094
};
\addlegendentry{$\mathbf{\hat{H}}_\mathrm{CC, interpolation}'$}
\addplot [thick, forestgreen4416044, mark=*, mark size=1, mark options={solid}]
table {%
0 146.538619995117
1 145.127227783203
2 143.616790771484
3 142.678405761719
4 141.571517944336
5 140.43196105957
6 139.686218261719
7 138.833572387695
8 138.280410766602
9 137.246597290039
10 135.924545288086
11 135.438446044922
12 134.337799072266
13 133.789627075195
14 132.761657714844
15 132.221008300781
16 132.040786743164
17 131.343597412109
18 130.995071411133
19 130.17854309082
20 129.13249206543
21 128.514389038086
22 127.870536804199
23 127.432373046875
24 126.896690368652
25 126.503112792969
};
\addlegendentry{$\mathbf{\hat{H}}_\mathrm{CC, nearestneighbor}'$}
\addplot [thick, crimson2143940, mark=*, mark size=1, mark options={solid}]
table {%
0 169.629531860352
1 162.217376708984
2 155.552917480469
3 152.708053588867
4 150.433975219727
5 147.729644775391
6 144.669143676758
7 142.697082519531
8 141.084365844727
9 139.145736694336
10 137.399505615234
11 136.502075195312
12 134.965850830078
13 133.443984985352
14 132.245361328125
15 131.807647705078
16 131.421966552734
17 130.673065185547
18 129.958541870117
19 129.344802856445
20 128.287445068359
21 127.426559448242
22 126.248023986816
23 125.369232177734
24 124.543739318848
25 123.61376953125
};
\addlegendentry{$\mathbf{\hat{H}}_\mathrm{Wiener}'$}
\end{axis}

\end{tikzpicture}

